Autocorrect in the Process of Translation -- Multi-task Learning Improves Dialogue Machine Translation

Automatic translation of dialogue texts is a much needed demand in many real life scenarios. However, the currently existing neural machine translation delivers unsatisfying results. In this paper, we conduct a deep analysis of a dialogue corpus and summarize three major issues on dialogue translation, including pronoun dropping (\droppro), punctuation dropping (\droppun), and typos (\typo). In response to these challenges, we propose a joint learning method to identify omission and typo, and utilize context to translate dialogue utterances. To properly evaluate the performance, we propose a manually annotated dataset with 1,931 Chinese-English parallel utterances from 300 dialogues as a benchmark testbed for dialogue translation. Our experiments show that the proposed method improves translation quality by 3.2 BLEU over the baselines. It also elevates the recovery rate of omitted pronouns from 26.09% to 47.16%. We will publish the code and dataset publicly at https://github.com/rgwt123/DialogueMT.

==> 04-testsets.tex <==
For better evaluation of \method, we  create a Chinese-English test set covering all translation issues, as discussed above. 
This section discusses the construction of the test set, including the rules and steps.

\subsection{Test Set Design}
We start from a TV drama subtitles corpus (the corpus we analyze in the second section). 
The reasons why we choose this corpus are twofold: 1) it is one of the few Chinese-English dialogue corpus that is big enough for us to select suitable dialogues; 2) the corpus is well pre-processed and contains wide-context information.

As we have analyzed, \droppro, \droppun and other translation challenges are common in this corpus. 
% Therefore we only require  to extract dialogues with such phenomena from the corpus.
Therefore we only extract dialogue samples featuring these three characteristics from the corpus.
However, there still exists several problems: 1) Most dialogues are too long and many of them require external scene knowledge for translation. 2) As shown in Table \ref{table_statistic-of-errors}, translation challenges are distributed sparse, hence randomly extracted dialogues are not conducive to evaluate. 3) The raw corpus does not contain typos, as verified manually.
% automatic label -> human extract -> add typos -> translate and label
To address these issues, we follow a 4-step process to construct the dialogue set.
\begin{enumerate}[itemsep=0 pt,topsep=0 pt]
    \item We first use automatic methods to detect potential dialogues with translation challenges to assist manual extraction. For \droppro, we detect the sentences with subject dropping. For \droppun, we simply use heuristic rules to make a rough selection, such as the Chinese  sentences with blanks. 
    \item Linguistic experts then start manual selection from the candidates automatically selected in the first step. Each manually selected dialogue follows such rules: 1) the dialogue should be able to present a complete scene independently; 2) the dialogue should contains at least one \droppro/\droppun challenge.
    \item To add \typo to the test set, we build a token-level Chinese typo table based on the test sets of a Chinese Spelling Check Task \cite{tseng2015introduction}. These are typos in real scenes and we have translated the original datasets into a version of simplified Chinese following \citet{wang2018hybrid}. We match Chinese tokens in the test set according to the table, and then verify and mark the sentences that are matched. We also try to ensure that the typos are not repeated.
    \item Finally,  linguistic experts translate the collected dialogues into English and annotate sentences that contain \droppro, \droppun or \typo challenges.  To ensure the quality of the test set, additional quality inspection process is also conduct. 
    %We don't tell them sentences that contain \droppro to avoid misleading. The translators need to understand the context of the dialogues. During translation, if they find that the pronoun that appears in the their translation does not appear in the original text, they are requested to label it as a \droppro sentence. They also need to explicitly provide the dropped pronouns in Chinese sentences and their translations in English. \droppun and \typo are also similarly labelled.
\end{enumerate}

Completing all the annotations, we  obtain a challenge test set. At the same time, we have $test_{gold}$ by recovering or repairing \droppro, \droppun and \typo according to human annotations.
%Several examples of our labelled dialogues are shown here\footnote{https://docs.google.com/document/d/19HS6hiHDptECCxrWr\\9COBE6qPsqsfFLD89w3BBIOjtQ/edit?usp=sharing}.


\begin{table}
\centering
\small
%\scriptsize
\begin{tabular}{|l|c|}
\hline
\textbf{Item}   & \textbf{Count} \\ \hline
\#dialogues & 300             \\
\#sentence pairs  & 1,931           \\
\#total tokens    & 19,155/15,976   \\
\#average tokens  & 9.92/8.27       \\
\#\droppro      & 299             \\
\#\droppun      & 542             \\
\#\typo    & 203             \\ \hline
\end{tabular}
\caption
{Statistics on the test set. ``/'' denote numbers in Chinese and English separately.}
\label{table_statistics}
\end{table}

\subsection{General Statistics}
Statistics on the built test set are displayed in Table \ref{table_statistics}. We show the number of dialogues, bilingual pairs, \droppro/\droppro/\typo, tokens, and the average number of tokens per sentence. 
Building such a test set is hard and time-consuming as we need to perform manual selection, translation and annotation. 
% The scale of this test set is not very large, because it is very challenging to build. The main difficulty is that most of them do not meet the requirements of expressing a complete scene. So manual judgment is required during extraction.
% Although sentences in the test suite are not very long, they are very hard to be correctly translated. It will be verified in our experiments. 

\subsection{Evaluation Metrics}
\label{section_testsets_evaluation}
We describe here how we evaluate dialogue translation quality on this test set in addition to using n-gram based metrics such as BLEU.
% As shown in Table \ref{table_general}, we will test from the overall and details aspects. 
For \droppun and \typo, we evaluate BLEU scores on sentences containing missing punctuation or typos according to the annotation information. As for \droppro, because we have annotated the missing pronoun in each \droppro sentence and its corresponding English translation during construction, and almost each sentence in our test set containing \droppro has no other explicit pronouns, we can judge if a tested model is able to successfully recover and translate dropped pronouns by checking whether dropped pronouns exist in translation. We evaluate the translation quality of the model for \droppro phenomenon by the percentage of correctly recovering and translating the dropped pronouns.

% All the results in Table \ref{table_general} are under the offline setting with all the context in the dialogue can be used.
All the results in Table \ref{table_general} are under the offline setting while all the context in the dialogue can be used.
We also evaluate results in online setting with different lengths of context in Table \ref{table_compare_context} and Figure \ref{pdf_offline}.

